A Conceptual Reference Model for Human as a Service Provider in Cyber Physical Systems

In Cyber Physical Systems humans are often kept in the loop as operators and/or service users. Yet in many cases, humans and machines collaborate and provide services to each other. Research on service models and service composition for CPS exist; however, humans as service providers have not been adequately considered as part of the CPS service composition model. We provide a classification of human-as-a-service in CPS, and we propose a Service Oriented Architecture (SOA) ontology model for the CPS environment as part of the Everything-as-a-Service paradigm. The model considers human characteristics and their dynamics, as a service provider or collaborator with the machine. As the ontology model is an enabler for engineering a self-adaptive CPS with human-machine collaboration as service providers, we describe how a commonly used self-adaptive reference model can be refined to benefit from the vision. We evaluate the ontological contribution against criteria that relates to accuracy, completeness, adaptability, clarity, and consistency. We demonstrate the feasibility of our conceptual reference model using a use case from the medical domain and we show how human-machine service provision is possible.

==> unused_files/new_ontology_self-adaptive.tex <==
\section{Using our Ontology in Self-adaptive HiLCPS}
The definition of our ontology is a pre-requiste for supporting future developments for a self-adaptive human-machine service provisioning in CPS. Self-adaptivity in HiLCPS can relate to bi-directional cooperation in which machines can help humans or vice versa. Therefore, it is essential to understand their behaviour to properly utilize their strengths in collaboration-oriented behaviour to obtain optimal results, not a competition to replace each other.

We instantiated the model using a simple scenario in the context of smart health care CPS environment. The CPS system connects patients, medical experts, and other smart agents (i.e. machines).  We  implemented the proposed model as semantic information model by leveraging OWL standard ontology language and Protege editor to evaluate the feasibility of our conceptual model. For simplicity, we do not provide instances of all concepts; only those essential to demonstrate our model proposal is feasible meets the evaluation criteria.

\subsection{Architecture}
Depending on the domain characteristics and requirements, several self-adaptation control-loop patterns can be used [lemos13], be it hierarchical control, master/slave, regional planner, or fully decentralized.

We show how our ontology model can enrich IBM's MAPE-K reference architecture using the Hierarchical Control pattern. In figure X, two layers of MAPE-K (Monitor-Analyze-Plan-Execute over
a shared Knowledge) feedback loop is implemented using the SOA paradigm. Although it looks like a master/slave pattern, in a hierarchical control pattern, the overall system is controlled by a hierarchical control structure where each hierarchy level has complete MAPE-K loops.

MAPE-K loops at different levels interact by exchanging information that contributes to new knowledge stored in a shared knowledge base that other hosts can access.

The top layer is a service broker that carries out service provisioning, composition, discovers and invokes service implementation candidates that meet the criteria requested and returns the best invocation result or composition plan to service consumer.

The second layer is self-adaptive systems with MAPE-K loops that interact directly with managed resources or subsystems. Depending on the service flow direction, each self-adaptive system at this hierarchical layer can be a Service Provider (when delivering services) and Service Consumer (when using services).

In service provisioning, the second layer coordinates with the adaptive service broker to achieve optimal results. The hierarchical structure allows the second layer to focus on more concrete adaptation goals, while the higher level can handle adaptation strategies for a broader perspective (Weyn 2013).




\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{pics/soa_sas_hierarchy.png}
\caption{SOA/MAPE-K hierarchical pattern}
\label{fig:autonomic}
\end{figure}


 %this need to be stated somewhere else too

\\\\


\subsection{Example Scenario}  
A health clinic uses a web chat as a health service channel. Patients can take advantage of this service to ask questions about clinical services, doctor schedules, book a GP, and get health advice.

In this scenario patient Adam, doctor David, and chatbot Cathy are layer two. Patients and doctors are represented by smart personal devices that provide an interface (e.g. API) for other entities to interact with their users.

Patient Adam accesses the webchat service to consult about the health problems he is experiencing. For every a new conversation session request, the chatbotService by Cathy chatbot is allocated first.

Cathy answers Adam's questions relying on its AI and knowledge from the local and shared knowledge base. During the conversation, Cathy acquires information from the chat with Adam and puts it on a shared knowledge base for others to use.

Adam repines of discomfort in his head, but Cathy's answers don't quite satisfy. With natural language processing and through its MAPE-K loops, Cathy detects Adam's emotions and upset. Cathy then sends a service discovery request to Service Broker with several criteria to maintain customer experience and satisfaction. Based on the conversation, Cathy can infer that Adam needs a service with better "Medicine and Dentistry", "Therapy and Counseling" knowledge and "Complex Problem Solving" skills which Cathy did not pose.  

Based on the criteria given by Service Broker discovers and invokes service implementation candidates that meet the invocation criteria using the SPARQL query as follows:
%PREFIX hcps:<http://www.semanticweb.org/user/ontologies/2020/11/untitled-ontology-9#>
\begin{lstlisting}[
    basicstyle=\footnotesize, %or \small or \tiny etc.
]
SELECT ?service ?skill ?knowledge ?capability
WHERE {
    ?service hcps:presents ?serviceprofile .
    ?serviceprofile hcps:hasProperty ?property .
    ?property hcps:includeCapability ?capability .
    ?capability hcps:hasHumanSkill ?skill .
    ?capability hcps:hasHumanKnowledge ?knowledge 
    FILTER (?skill=hcps:Complex_Problem_Solving && 
    ?knowledge=hcps:Medicine_and_Dentistry)
}
\end{lstlisting}
The query above returns the result that the chatDoctor service by doctor David is a suitable candidate. The service broker invokes the chatDoctor service for Cathy, which then gives David access to join the chat session. At this point, Cathy becomes a service consumer (for David) as well as a service provider (for Adam).

The doctor provides an \textit{adaptation service} for the chatbot to provide a better quality of service in the future. $Cathy$ the chatbot acquires the knowledge from the conversation between patient $Adam$ and doctor $David$. This knowledge can be in the form of questions, answers and responses given. 

David gives some advice to Adam, and they agree on a schedule for offline meetings. Adam, who was initially upset, ends the session with good satisfaction.

The instantiation of this scenario is shown in figure \ref{fig:sec2_instant}.

\begin{figure}[H]
\centering
\includegraphics[width=0.48\textwidth]{pics/scenario2_ontograf.png}
\caption{Individuals and classes relationships for Scenario 2.}
\label{fig:sec2_instant}
\end{figure}

By involving chatbot Cathy, doctor David can get other work done, handle more customers, thus increase productivity. Cathy can learn from David to provide more human responses by showing empathy. Meanwhile, Cathy can also offer answer suggestions to David, especially when it comes to data processing where humans are inferior to AI. 

This scenario shows that machines and humans can help each other extend the capabilities of both. Self-adaptive HiLCPS benefiting from our ontology can modify its behaviour or structure in response to the changing context (environment, goal, system) that they perceive.

==> unused_files/old_discussion.tex <==
Working with humans makes HiLCPS different from traditional CPS. There are three things that distinguish HiLCPS from traditional CPS, namely cognition, predictability, and motivation \cite{Sowe2016cphs}. In terms of cognition, the different ways in which people and computers observe, process, and act present challenges (and opportunities) for people to work together with computers to achieve a goal best. In terms of predictability, people are more dynamics; they do not perform the task the same way every time. Their performance improves by experience but can also deteriorate due to distractions. Lastly, motivation; unlike computing systems, human work is driven by motives. Motivations vary widely from financial incentives, compliments, or other forms of rewards

\subsection{Human-Machine Service Provisioning}
Humans and machines have different abilities in processing information and dealing with uncertainties. Machines are suitable for both repetitive and static tasks. Humans are more adaptive, so they are better suited for dynamic tasks. Human behaviour is naturally theological, which changes dynamically influenced by intention, intuition, and experience \cite{rasmussen1983skr, Lavazza2018Dec}. In contrast to other machines/artificial systems where the teleology property arises because the designer programs it. 
Therefore, task allocation between humans and machines is very challenging as it must pay attention to the strengths and weaknesses of each. 

Rasmussen \cite{rasmussen1983skr} classified human behaviour into three types of information processing behaviours, namely \textit{Skill behaviour}, \textit{Rule behaviour}, and \textit{Knowledge behaviour}. \textbf{Skill-based behaviour} is a sensory-motor activity carried out automatically without conscious control, which is a highly integrated pattern. The next level is \textbf{Rule-based behaviour}, which is a composition or work sequence in a familiar environment referring to stored rules or procedures obtained from previous experiences, instructions (e.g. cooking recipes), or the results of previous planning. Next is \textbf{Knowledge-based behaviour} that appears when facing unfamiliar situations where there are no know-how, rules, procedures that can be used so that performance is more goal-oriented by using several alternative plans and considerations of the consequences.

Building on what Rasmussen proposed, Cummings \cite{cummings2014man} added another category called \textbf{Expertise-based Behaviour}. Expertise-based behaviour arises because knowledge exercised by uncertainties in very different conditions so that a person may evolve from being knowledge-able to become an expert. Uncertainty arises when dealing with many unknown variables so that the situation could not be fully determined due to lack of information. It can arise from exogenous sources coming from outside the system, or endogenous sources from within the system.

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{pics/human_machine_allocation.png}
\caption{Role allocation base on the level of uncertainty . Adopted from \cite{cummings2014man}} \label{fig:human_machine_alloc}
\end{figure}

Figure \ref{fig:human_machine_alloc} maps those four types of information processing behavior against human-machine information processing capability towards uncertainty. One approach is to classify each of the existing tasks in HiLCPS into these four categories and carry out a task allocation based on Cummings' suggestions. Skill-based tasks are the best candidates for automation if reliable sensors and feedbacks support them. If the rule/procedure set is mature and tested, automation can be applied to the Rule-based tasks. For the  Knowledge-based tasks, automation can be used to help organize and synthesize data. Expertise-based tasks comes with high uncertainties so that human reasoning is superior; automation can be used as a tool or partner.

Nevertheless, task allocation must also pay attention to other aspects such as costs, budget, service limitations, human performance factors, QoS constraints, and so on. These challenges must be taken into consideration by service orchestrators in human-machine service provisioning of HiLCPS. 

\subsection{Level of Automation}
The level of automation can be used to measure the extent to which humans and machines are involved in completing tasks. In manufacturing, the level of automation can be defined as "the allocation of physical and cognitive tasks between humans and technology, described as a continuum ranging from totally manual to totally automatic" \cite{frohm2008levels}.

A quantitative measure of automation level must consider the weight for each task where this weight should be determined based on the level of complexity, difficulty, and criticality. Level of Automation ($LoA$) is defined using a simple weighting scheme which is a function of the number of automated tasks \cite{wei1998loa}, as follows:

\begin{equation}
 LoA=1-\frac{\sum_{i=1}^{N} t_iw_i}{\sum_{i=1}^{N} w_i} \label{eq:1}  
\end{equation}

where $t_i$ is a task indicator which has a value of 0 if the task $i$ is done by a machine (automated), and has a value of 1 if the task $i$ is done manually or by a human; while $N$ is the total number of tasks.

The uncertainty level will determine how complex the information will be processed, how difficult decisions can be made, and the criticality for many cases. So we propose to apply weights toward tasks based on their categories (see figure 1) from low to high for Skill-based, Rule-based, Knowledge-based, Expertise-based, sequentially. Thus, the Equation \eqref{eq:1} can be rewritten as:
\begin{equation}
 LoA=1-\frac{\sum_{i=1}^{N} (t_iw_i^s+t_iw_i^r+ t_iw_i^k+t_iw_i^e)}{\sum_{i=1}^{N} (w_i^s+w_i^r+w_i^k+w_i^e)}   
\end{equation}
in which
$w^s$ is the weight for Skill-based task,
$w^r$ is the weight for Rule-based task,
$w^k$ is weight for Knowledge-based task,
and $w^e$ stand for the weight for Expertise-based task.

\subsection{Trust Calibration}
Trust is an attitudinal judgment of the degree to which a user can rely on an agent to achieve their goals under uncertainty conditions. In the scope of human-machine service, the user is the service composer or task allocator who determines whether a machine or a human performs a task. In Skill-based and Rule-based tasks where the machine should be reliable, having an LoA that is too high can mean over-trust, where the user overestimates the machine's reliability. However, having a very LoA can indicate under-trust, which will result in low machine utilization.
In Knowledge-based and Expertise-based humans seem superior with their adaptability. However, humans have the threat of permanent shaping factors (e.g. fatigue, mood, stress, etc.) that need to be anticipated. To achieve optimal human-machine collaboration, keeping proper trust calibration is needed because poor trust calibration could lead to safety issues.

==> unused_files/old_ibm_autonomic_computing.tex <==
We should how our IBM autonomic reference architecture can be enriched using our ontology. IBM model  identifies five building blocks for an autonomic system \cite{computing2006architectural}: manual manager, autonomic manager, touchpoint, knowledge sources, and enterprise service bus. As shown in figure \ref{fig:autonomic}, the autonomic system architecture can be described in terms of Human-in-the-Loop CPS (HiLCPS) as follows:



\textbf{The manual manager} is the implementation of a user-interface where humans can carry out management functions manually. At this layer, humans evaluate and justify current operating procedures and adaptation strategies and then delegate them to the autonomic managers. Managers can determine what conditions and tasks, human intervention is required or when machines should be relied on to complete tasks. This layer can be realized in our model as an adaptation service provided by humans with authorized executive/managerial roles.

\textbf{The autonomic manager} is an autonomous component that implements a control loop that includes monitoring, analyze, plan, execute, and share knowledge (MAPE-K) functions. In CPS, this component is manifested in the Cyber layer. There are two kinds of autonomic manager functions. First, Touchpoint autonomic managers implement intelligent control loops to automate combinations of the tasks to provide self-* properties. Touchpoint autonomic manager  through their touchpoints to oversee the managed resources.

The second is the orchestration-autonomic managers in charge of orchestrating Touchpoint autonomic managers within single or multi-discipline and across domains. Autonomic managers use knowledge from internal and external sources (e.g. using other ontologies) to perform management functions that contribute to new knowledge. Our proposed model assists adaptation by providing diverse knowledge, not only relying on machines but also validated by humans.  Our human capability model provides a vital knowledge structure for determining which humans to be involved in achieving goals. So that ultimately the autonomic manager can find the optimal configuration for human-machine service provisioning.

\textbf{Touchpoint} is a block where sensors, effectors, and actuators are in direct contact with managed resources (e.g. environment, storage, etc.). We propose a Touchpoint as a physical layer in CPS that involves human services, not just machines, as sensors or actuators. As a sensor, the Touchpoint observes the managed resources and sends information to the layer above (i.e. autonomic/manual manager). As an effector, Touchpoints run the policies set by the manager towards themselves and managed resources. Having a human component at the Touchpoint provides additional flexibility for the system that is not limited to machine capabilities.

\textbf{Knowledge source} is the implementation of a registry, knowledge base, or other forms of repository according to architectural requirements. In SOA, we have a service repository to hold information about the behavior and interfaces of services presented in the service profile (figure \ref{fig:service_profile} or service capability ontology (figure \ref{fig:human_capability}) which is linked to other relevant knowledge bases. This knowledge is shared, arranged across layers, inferred from managed resources as unstructured/structured data, obtained as information, organized as knowledge to gain wisdom at its peak.The source of knowledge is not only from within the system but also from external sources. Every individual in the system, humans and machines, can contribute to new knowledge. The autonomous manager processes the data collected by Touchpoint as useful information stored in the knowledge base for further adaptive planning. Manual managers can express their tacit knowledge as explicit knowledge in the knowledge base.



%Knowledge, organized according to syntax and semantics, is useful for reasoning, decision making, determining policies, and adaptation plans. In the autonomic system, knowledge plays a vital role in making decisions, mainly to deal with uncertainty. 



All of the above building blocks are integrated by the \textbf{Enterprise Service Bus} to build autonomous systems.

The IBM architecture blueprint emphasizes the human role in the manual manager. We argue that
humans can also be involved in the Touchpoint layer along with autonomous machines. Apart from completing the gaps resulting from machines' limitations, humans can also help machines perform better tasks and vice versa.


==> unused_files/old_scenario.tex <==
\section{Case Study : Smart Healthcare}
 We instantiated the model using two scenarios in the context of smart health care CPS environment. The CPS system connects patients, medical experts, and other smart agents (i.e. machines). We  implemented the proposed model as semantic information model by leveraging OWL standard ontology language and Protege editor to evaluate the feasibility of our conceptual model. For simplicity, we do not provide instances of all concepts; only those essential to demonstrate our model proposal is feasible meets the evaluation criteria.
\\\\


\textbf{Scenario 2:}  Adam, a patient, wants to consult about his health via a chat service. A Cathy, a chat bot, was assigned to answer Adam's questions. However, the system detects that Adam is not satisfied with Cathy's answer; Adam needs a service with better "Medicine and Dentistry" knowledge and "Complex Problem Solving" skills which Cathy does not pose. using the SPARQL query as follows:
%PREFIX hcps:<http://www.semanticweb.org/user/ontologies/2020/11/untitled-ontology-9#>
\begin{lstlisting}[
    basicstyle=\footnotesize, %or \small or \tiny etc.
]
SELECT ?service ?skill ?knowledge ?capability
WHERE {
    ?service hcps:presents ?serviceprofile .
    ?serviceprofile hcps:hasProperty ?property .
    ?property hcps:includeCapability ?capability .
    ?capability hcps:hasHumanSkill ?skill .
    ?capability hcps:hasHumanKnowledge ?knowledge 
    FILTER (?skill=hcps:Complex_Problem_Solving && 
    ?knowledge=hcps:Medicine_and_Dentistry)
}
\end{lstlisting}

The instantiation of this scenario is shown in figure \ref{fig:sec2_instant}.

\begin{figure}[H]
\centering
\includegraphics[width=0.48\textwidth]{pics/scenario2_ontograf.png}
\caption{Individuals and classes relationships for Scenario 2.}
\label{fig:sec2_instant}
\end{figure}

In this scenario, the doctor provides an \textit{adaptation service} for the chatbot to provide a better quality of service in the future. $Cathy$ the chatbot acquires the knowledge from the conversation between patient $Adam$ and doctor $David$. This knowledge can be in the form of questions, answers and responses given. Machines can learn from humans to provide more human responses by showing empathy. Meanwhile, machines can also offer answer suggestions to humans, especially when it comes to data processing where humans are inferior to AI. Machines and humans can help each other extend the capabilities of both.



\textbf{Scenario 1:} The Cardiac output monitoring machine, $EcgDev$, installed on $Andy$'s patient, in $siteA$, its loses signal. Therefore, $EcgDev$ seek for officers nearby with the skills "Cardiac output CO monitoring units or accessories" to immediately take the necessary emergency measures, such as device actuation or emergency care for patient Andy. $Sisy$ is a "Critical Care Nurse" who offers an \textit{actuating service} $actuatingBySisy$ that relies to the sensors and the interface provided by her smartphone to retrieve notification and context. As soon as the notification was received, Sisy rushed to the location where the requester is located. 

\begin{figure}[H]
\centering
\includegraphics[width=0.48\textwidth]{pics/scenario1_ontograf.png}
\caption{Individuals and classes relationships for Scenario 1.}
\label{fig:sec1_instant}
\end{figure}

This scenario can be instantiated into ontology as shown in figure \ref{fig:sec1_instant}. $Andy$ and $Sisy$ are individuals (i.e. instances) of the Human class, whereas $EcgDev$ is an individual of Machine class. $Sisy$ has a human capability represented by a technology skill "Cardiac output CO monitoring units or accessories" to operate $EcgDev$. The machine capability that determines the operational characteristics of $EcgDev$ in this figure is its specifications (e.g. ECG sensor, ECG firmware). Both $Andy$, $Sisy$, and $EcgDev$ share the same context, namely the location $siteA$.

By using this instantiation, one can find the available human service (i.e. $actuatingBySisy$) on Service Discovery by executing the SPARQL to traverse the Service Profile as follows:

\begin{lstlisting}[
    basicstyle=\footnotesize, %or \tiny or \small \footnotesize etc.
]
SELECT ?service
WHERE {
    ?service hcps:presents ?serviceprofile .
    ?serviceprofile hcps:hasProperty ?property .
    ?property hcps:includeCapability ?capability .	
    ?property hcps:includeContext ?context .
    ?capability hcps:hasHumanSkill ?skill .
    FILTER (?context=hcps:siteA  &&
    ?skill=hcps:Cardiac_output_CO_monitoring_units
    _or_accessories)
}
\end{lstlisting}

In this scenario, machines involve humans to perform beyond their abilities/functionalities. If it turns out that $EcgDev$ does not raise a false alarm, it will receive a favourable rating of $Sisy$, vice versa. This rating system in the future will determine whether the machine $EcgDev$ needs to be repaired or even replaced. Conversely, $EcgDev$ can also give a nurse $Sisy$  a positive rating for her responsiveness.
